The Limit of Recursion in State-based Systems

We prove that omega^2 strictly bounds the iterations required for modal definable functions to reach a fixed point across all countable structures. The result corrects and extends the previously claimed result by the first and third authors on closure ordinals of the alternation-free mu-calculus in [3]. The new approach sees a reincarnation of Kozen's well-annotations, devised for showing the finite model property for the modal mu-calculus. We develop a theory of 'conservative' well-annotations where minimality of annotations is guaranteed, and isolate parts of the structure that locally determine the closure ordinal of relevant formulas. This adoption of well-annotations enables a direct and clear pumping process that rules out closure ordinals between omega^2 and the limit of countability.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Alexis Saurin (Editor): Fixed Points\\ 
in Computer Science 2024 (FICS 2024).\\
EPTCS 435, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.435.1}{10.4204/EPTCS.435.1}}

